Massive Choice, Ample Tasks (MaChAmp): A Toolkit for Multi-task Learning in NLP

Transfer learning, particularly approaches that combine multi-task learning with pre-trained contextualized embeddings and fine-tuning, have advanced the field of Natural Language Processing tremendously in recent years. In this paper we present MaChAmp, a toolkit for easy fine-tuning of contextualized embeddings in multi-task settings. The benefits of MaChAmp are its flexible configuration options, and the support of a variety of natural language processing tasks in a uniform toolkit, from text classification and sequence labeling to dependency parsing, masked language modeling, and text generation.

==> conclusion.tex <==
We introduced \name{}, a powerful toolkit for multi-task learning supporting a
wide range of NLP tasks. We also provide initial experiments demonstrating the
usefulness of some of its options. We learned that multi-task learning is
mostly beneficial for setups in which multiple datasets are annotated for the
same set of tasks, and that dataset embeddings can still be useful when
employing contextualized embeddings. However, the current experiments are just
scratching the surface of \name{}'s capabilities, as a wide variety of tasks
and multi-task settings is supported.


